Exploring Interference between Concurrent Skin Stretches

Proprioception is essential for coordinating human movements and enhancing the performance of assistive robotic devices. Skin stretch feedback, which closely aligns with natural proprioception mechanisms, presents a promising method for conveying proprioceptive information. To better understand the impact of interference on skin stretch perception, we conducted a user study with 30 participants that evaluated the effect of two simultaneous skin stretches on user perception. We observed that when participants experience simultaneous skin stretch stimuli, a masking effect occurs which deteriorates perception performance in the collocated skin stretch configurations. However, the perceived workload stays the same. These findings show that interference can affect the perception of skin stretch such that multi-channel skin stretch feedback designs should avoid locating modules in close proximity.

==> Previous_Versions/Introduction_Ying.tex <==
\section{INTRODUCTION}
Proprioception, the sense of limb position relative to the body \cite{tuthill2018proprioception}, is essential for coordinating human movements, especially in tasks involving multiple joints \cite{sainburg1993loss} and limbs \cite{Schaffer2021Ararecase, kazennikov2005goal}, such as walking or driving. However, this sensory feedback is absent when operating an artificial limb, such as a tele-operated robot or prosthetic, and its loss has been shown to reduce operator performance and increase workload \cite{schiefer2018artificial, papaleo2023integration}. Providing supplementary proprioceptive feedback through somatosensation aids in incorporating artificial limbs into tasks and the user’s body schema \cite{papaleo2023integration, blank2008identifying}. However, the capacity of users to exploit this added information is not yet completely understood.

To evaluate the benefits of providing supplementary proprioception feedback to users of artificial limbs, several modalities have been proposed, including vibrotactile \cite{noccaro2020ANovelProprioceptive, pinardi2021Cartesian, alva2020wearable}, electrotactile \cite{boljanic2022design}, and skin stretch \cite{wheeler2010investigation}. Vibrotactile and electrotactile feedback, which stimulate the somatosensory system through vibration and electrodermal activity, are physically compact and lightweight, facilitating easier integration with robotic systems \cite{enami2024ASurvey}. However, skin stretch, which mimics natural proprioception mechanisms by stretching the skin \cite{tuthill2018proprioception}, has been shown to result in lower error rates compared to other modalities \cite{bark2008comparison}, making it an especially attractive option for providing intuitive and accurate feedback.

Proprioceptive information, such as limb posture, is inherently multi-dimensional. However, skin stretch feedback devices have typically been designed to convey only one dimension of this information \cite{clark2018rice, bark2009wearable, schorr2013sensory}. To communicate higher-dimensional information through skin stretch, the common approach has been to increase the number of skin stretch channels, with recent applications providing 3-dimensional \cite{chinello2016design, chinello2017design} and 4-dimensional feedback \cite{yem2015development}. While these devices have shown some ability to convey multi-dimensional information, the effect of increasing the number of channels on skin stretch perception has only been explored in preliminary studies \cite{zook2019effect}. In this study, it was found that concurrent squeezing can interfere with skin stretch perception.

Since the skin is a continuous and deformable membrane, its deformation must be processed by the brain. Therefore, the activation of one skin stretch device may interfere with the perception of another when two devices are used simultaneously. This phenomenon has been observed in vibrotactile \cite{craig1995vibrotactile} and electrotactile \cite{krishnasamy2023effect} scenarios when multiple simultaneous stimuli overlap. However, the interference effect between skin stretch devices has not been thoroughly investigated. Additionally, the impact of the placement of additional channels on interference is unclear, as most multi-channel skin stretch devices apply skin stretches in close proximity \cite{chinello2016design, chinello2017design, yem2015development}.


This study addresses the following research question: {\em What is the impact of applying two skin stretches simultaneously on the perception and intuitiveness of skin stretch}? To investigate the interference effect and its implications for multi-channel skin stretch feedback systems, we conducted a user study involving 30 participants. They were simultaneously stimulated by two skin stretch modules across two attachment configurations and varying intensity levels. Our findings provide insights into how simultaneous stimuli influence perception and performance.
